A Scalable Inference Method For Large Dynamic Economic Systems

The nature of available economic data has changed fundamentally in the last decade due to the economy's digitisation. With the prevalence of often black box data-driven machine learning methods, there is a necessity to develop interpretable machine learning methods that can conduct econometric inference, helping policymakers leverage the new nature of economic data. We therefore present a novel Variational Bayesian Inference approach to incorporate a time-varying parameter auto-regressive model which is scalable for big data. Our model is applied to a large blockchain dataset containing prices, transactions of individual actors, analyzing transactional flows and price movements on a very granular level. The model is extendable to any dataset which can be modelled as a dynamical system. We further improve the simple state-space modelling by introducing non-linearities in the forward model with the help of machine learning architectures.

==> Background/kalman.tex <==

%\paragraph{Kalman Filter}
% Kalman Filtering \cite{kalman1960general} is applied to obtain an optimal weighted average of the background (forecast) data and observations to effectively deal with the uncertainty.
%The weighted average, known as Kalman Gain ($\boldsymbol{K}$) is used to improved a posteriori estimate from the prior estimate i.e $\boldsymbol{x_t}$ given $\boldsymbol{y_{1},\dots,y_t}$.
%The Kalman equations can then be derived by using a Maximum a Posteriori estimation, analytically solving the cost function. 

%At time $t-1$, the knowledge of the system is summarised by the posterior distribution 
%$$
%\mathbf{x_{t-1}}|\mathbf{y_{t-1}},\mathbf{x^b_{t-1}} \sim \mathcal{N}(\mathbf{x^a_{t-1}},\boldsymbol{P_{t-1}})
%$$
%Equations in Kalman filter follow a prediction-correction methodology \cite{aschDataAssimilationMethods2016} with the weight matrix, Kalman Gain, 
%$$\boldsymbol{K_t = P^f_t M^T _t(H_{t}P^f_{t}M^T_{t} + R_t)^{-1} }$$
% \useshortskip
% \begin{equation} \label{eq1}
% \begin{split}
% J(\mathbf{x^a_t}) &= (\mathbf{x_t}-\mathbf{x^b_t})^{\mathrm{T}}\mathbf{Q_t}^{-1}(\mathbf{x_t}-\mathbf{x^b_t}) + (\mathbf{y_t}-\mathcal{H}(\mathbf{x_t}))^{\mathrm{T}}\mathbf{R_t}^{-1}(\mathbf{y_t}-\mathcal{H}(\mathbf{x_t})) \\
% &= \mathbf {J_b(x_t) + J_o (x_t)}
% \end{split}
% \end{equation}
%Kalman Gain is used to update the previously predicted states $\boldsymbol{x^f}$ and $\boldsymbol{P^f}$ to analysis value $\boldsymbol{x^a}$ and $\boldsymbol{P^a}$ respectively. The correction keeps on reducing the state error covariance, P.
%\begin{equation*}
%\boldsymbol{x^a_t = x^f_t + K_t (y_t - Hx^f_t)}
 % \quad\quad 
%\boldsymbol{P^a_t = (I - K_t H_t)P^f_t}
%\end{equation*}
% Equations in Kalman filter follow a prediction-correction methodology  \cite{aschDataAssimilationMethods2016}.

% \underline{\textbf{Prediction}}: Propogate current state forward using linear model operators : 
% \useshortskip
% \begin{myequ}
% \boldsymbol{x^f_{t}} = \boldsymbol{M_{t-1}x^a_{t-1}}
%   \quad\quad 
%  \boldsymbol{P^f_{t}} = \boldsymbol{M_{t-1}P_{t-1}M^T_{t-1}} + \boldsymbol{Q_{t-1}} 
% \end{myequ}

% where M is the linear state operator, $P_{t-1}$ is the previous estimated state error covariance and $Q_{t-1}$ is background error covariance matrix.
% \\
% \underline{\textbf{Kalman Gain}}: 
% Calculating the Kalman Gain based on R, the measurement error ; linear H operator to map observation to state and $\boldsymbol{P^f}$ obtained above.
% $$
% \boldsymbol{K_t = P^f_t M^T _t(H_{t}P^f_{t}M^T_{t} + R_t)^{-1} }
% $$
% \underline{\textbf{Correction}}: 
% The Kalman Gain is used to update the $\boldsymbol{x^f}$ and $\boldsymbol{P^f}$ to analysis value $\boldsymbol{x^a}$ and $\boldsymbol{P^a}$ respectively. The correction keeps on reducing the state error covariance, P.

% \begin{myequ}
% \boldsymbol{x^a_t = x^f_t + K_t (y_t - Hx^f_t)}
%   \quad\quad 
% \boldsymbol{P^a_t = (I - K_t H_t)P^f_t}
% \end{myequ}

% Feedback loop is repeated until all observations have been used. 

% \begin{figure}[H]
%     \centering
%     \includegraphics[scale=0.75]{Background/Kalman.png}
%     \caption{ Kalman Filtering intuition \cite{berryIntroductionDataAssimilation}}
%     \label{fig:my_label}
% \end{figure}

==> kalman_alog.tex <==
\begin{algorithm}[H]
\begin{algorithmic}[1]
\STATE Initialise Priors $Q_0, R_{0}, F, \beta_{0}, \sigma$
\FOR{t=1...T} 
    \STATE \underline{Prediction Step}
    \STATE{$\beta_{t-1} = F \beta_{t-1}$}
    \STATE{$Q_{t-1}=F Q_{t-1} F'$}

    \STATE \underline{Updating Step}
    \STATE{$K_t =Q_{t-1} x_t' (x_t Q_{t-1}x_t'+\sigma_t^2)^{-1} $} \COMMENT{Gain Matrix}
    \STATE{$\beta_{t} = \beta_{t-1} + K_{t}(y_t-x_t \beta_{t-1})$} \COMMENT{Posterior Mean of $\beta_t$}
    \STATE{$Q_{t} = (I - K_t x_t) Q_{t-1}$} \COMMENT{Posterior Variance of $\beta_t$}
\ENDFOR

\end{algorithmic}
%\caption{A generalized description of the STATE space model incorporating stochastic volatility estimates}
\caption{Modified TVP-VAR-DA algorithm}
\label{algo1}
\end{algorithm}










